Robust GANs against Dishonest Adversaries

Robustness of deep learning models is a property that has recently gained increasing attention. We explore a notion of robustness for generative adversarial models that is pertinent to their internal interactive structure, and show that, perhaps surprisingly, the GAN in its original form is not robust. Our notion of robustness relies on a perturbed discriminator, or noisy, adversarial interference with its feedback. We explore, theoretically and empirically, the effect of model and training properties on this robustness. In particular, we show theoretical conditions for robustness that are supported by empirical evidence. We also test the effect of regularization. Our results suggest variations of GANs that are indeed more robust to noisy attacks and have more stable training behavior, requiring less regularization in general. Inspired by our theoretical results, we further extend our framework to obtain a class of models related to WGAN, with good empirical performance. Overall, our results suggest a new perspective on understanding and designing GAN models from the viewpoint of their internal robustness.

==> cifar_section.tex <==
\subsection{CIFAR10}\label{supp:cifar_exp}
Finally, we perform our empirical analysis on the CIFAR10 data. Here, our adversary is
 \begin{align*}
\Phi(D(x)) = \left\{\begin{array}{llll}
1-D(x) & \;\text{with probability $0.1$}\\
\sqrt{D(x)}&\;\text{with probability $0.1$}\\
(D(x))^2&\;\text{with probability $0.2$}\\
D(x) & \;\text{otherwise},
\end{array}\right.\end{align*}
 For this set of experiments, recall our assumptions in Section~\ref{sec:robust}: (1) Access to an optimal discriminator $D$; and (2) with access to an optimal $D$, the model is able to learn the corresponding optimal generator, leading e.g. to successful lerning without an adversary.
While these assumptions are reasonable for relatively easy tasks (and, as in Gaussian and MNIST experiments, lead to the expected results), on more complex tasks factors such as the optimization algorithm and data properties may play a role too.

\begin{figure}[htp]
%\vspace{-0.2in}
 \centering
   \includegraphics[width=5.5in]{cifar_sample_horizontal.pdf}
   %\vspace{-0.2in}
   \caption{Example results on CIFAR10 (no clipping).}\label{fig:cifar_sample}
   \vspace{-0.15in}
 \end{figure}
 \begin{figure}[htp]
%\vspace{-0.2in}
 \centering
   \includegraphics[width=5.5in]{cifar_plot_horizontal}
   %\vspace{-0.2in}
   \caption{Discriminator's outputs. 
   %The blue points represent the outputs for the true data, while the red points represent the outputs for the generated data. 
   Upper right: the extreme behavior of $D$, in addition to the adversary, can easily causing exploding or vanishing gradients in numerical experiments.}\label{fig:cifar_plot}
   %\vspace{-0.2in}
 \end{figure}

 Figure \ref{fig:cifar_sample} displays example images generated by the standard GAN and one of the robust models. Surprisingly, from a human viewpoint, it seems that with or without the adversary, both models learn to generate images that resemble CIFAR10 data. However, the plots of $D$'s outputs in Figure \ref{fig:cifar_plot} suggest a different story that also differs from the previous experiments. Even without the adversary, $D$ tends to output extreme values: the CIFAR10 data are assigned probabilities close to 1 while the generated data are assigned negligible probabilities. Although the plots seem to suggest there is some learning in the beginning, $D$ starts to produce extreme values before a similar distribution has been learned by $G$. The extreme behavior of $D$ contradicts any strong evidence that the models approximately learn the data distribution. One conjecture to reconcile the strong discriminator with the visual results is that $D$ focuses on low-level perturbations off the image manifold that are less perceptible by the human eye \cite{jo17,guo18}.
 
Good performance on high-dimensional images often requires some stabilizing modifications of the training algorithm \citep{gulrajani2017improved,miyato2018spectral,karras2018progressive}. We conjecture that those modifications, just like clipping, improve the robustness of the models. %\sj{would be really good to have some results on that, even for some of these -- an obvious reviewer question} 
These methods also probably change the space of functions parameterized by the network. Incorporating the effect of these modifications, and the data properties, into a full theoretical analysis is an interesting avenue of future work.

 

\iffalse

The previous two experiments have demonstrated the effectiveness of our robust frameworks. It might be tempting to expect such a behavior to continue as we move to harder and harder data. Let us first emphasize the assumptions we have made to derive the theory: (1) {Access to an optimal $D$;} (2) Inherently, with the access to an optimal $D$, the model should be able to learn the true distribution without the adversary, after which we can then evaluate its robustness with the presence of an adversary. 

For the previous two experiments, the task is relatively easy and we do expect the above assumptions to hold approximately (as also observed from the results). %
%: discriminating two-dimensional Gaussian data or a black-while digit from initially randomly generated data should not be hard; and we indeed see that the model reasonably learn to generate similar data when there is no adversary. 
For high-resolution image data, it may be too optimistic to hope that the assumptions will still hold, and in this section, we would like to investigate such a limit of our theory and motivate future research. 
As an example, we show the results for CIFAR10 in the following. %Similar results have been observed in other datasets. 
The adversary we will apply is 
 \begin{align*}
\Phi(D(x)) = \left\{\begin{array}{llll}
1-D(x) & \;\text{with probability $0.1$}\\
\sqrt{D(x)}&\;\text{with probability $0.1$}\\
(D(x))^2&\;\text{with probability $0.2$}\\
D(x) & \;\text{otherwise},
\end{array}\right.\end{align*}
\begin{figure}[htp]
%\vspace{-0.2in}
 \centering
   \includegraphics[width=3.2in]{fig/cifar_sample.pdf}
   \vspace{-0.2in}
   \caption{Example results on CIFAR10 (no clipping).}\label{fig:cifar_sample}
   \vspace{-0.2in}
   \includegraphics[width=3.2in]{fig/cifar_plot.pdf}
   \vspace{-0.2in}
   \caption{Discriminator's outputs. 
   %The blue points represent the outputs for the true data, while the red points represent the outputs for the generated data. 
   Upper right figure: less data points because the extreme behavior of $D$, in addition to the adversary, can easily causing exploding or vanishing gradients in numerical experiments.}\label{fig:cifar_plot}
   \vspace{-0.2in}
 \end{figure}
 \begin{figure}[htp]
%\vspace{-0.2in}
 \centering
   \includegraphics[width=3.2in]{fig/cifar_plot.pdf}
   \vspace{-0.2in}
   \caption{Discriminator's outputs. 
   %The blue points represent the outputs for the true data, while the red points represent the outputs for the generated data. 
   Upper right figure: less data points because the extreme behavior of $D$, in addition to the adversary, can easily causing exploding or vanishing gradients in numerical experiments.}\label{fig:cifar_plot}
   \vspace{-0.2in}
 \end{figure}

Figure \ref{fig:cifar_sample} displays some images generated by the vanilla GAN and one of the robust model. Surprisingly, from the viewpoint of a human, it seems that with or without the adversary, both models learn to generate images that resembles CIFAR10 data. However, if we look at the plots of $D$'s outputs in Figure \ref{fig:cifar_plot}, the story is quite different from what we have in the previous experiments. Even without the adversary, $D$ tends to output extreme values for the data: the CIFAR10 data are assigned with probabilities close to 1 while the generated data are assigned negligible probabilities. Although the plots seem to suggest there is some learning in the beginning, it is reasonable to argue, based on the extreme behavior of $D$, that there is no strong evidence that the models approximately learn the data distribution. That is, the assumptions are unlikely to be satisfied, and this leads to the results that our current theory are unable to address. In fact, on complex image data, whether GAN actually learns the data distribution remains an open question, and it is often the case that for image data, $D$ tends to be too powerful. Most of the state-of-the-art results then require a more sophisticated training algorithm (i.e., regularization) \citep{gulrajani2017improved,miyato2018spectral,karras2018progressive}. \sj{would be really good to have some results on that, even for some of these -- an obvious reviewer question} We conjecture that like clipping, those training methods should also help to increase the robustness of the underlying model. In addition, those methods are likely to change the space of functions parameterized by the network. As such, How to incorporate the practical aspects into the theory and quantify the loss of robustness when ideal assumptions cannot be satisfied are interesting and immediate future directions.       %To summarize, when the assumptions are approximately met, we have successfully verified our theory. 
%How to incorporate the practical aspects into the theory and quantify the loss of robustness when ideal assumptions cannot be satisfied are interesting and immediate future directions.       
% \begin{figure}[H]
% \vspace{-0.8in}
%  %\centering
%  \hspace{-0.2in}
%    \includegraphics[width=6in]{fig/mnist_1.pdf}
%    \vspace{-0.8in}
%    \caption{First row: success rate v.s. clipping value (success = learn digits. Actually, the architecture is very good in the sense that all the models either learn a roughly uniform distribution over the digits (see the plots for TV distance) or completely learn nothing (loss becomes nan)); Second row: averaged TV distance to the uniform distribution for the successful runs}\label{fig:mnist_1}
%    \vspace{-0.2in}
%  \end{figure}

\fi

==> empirical_workshop.tex <==
{\section{Empirical Results: Robustness}
To probe our theoretical results in practice, we empirically evaluate the robustness of the models in Section \ref{sec:robust}. We select several models from our robust class and verify their internal robustness. We generally observe that these models are also empirically more robust to perturbations and, in addition, they tend to train more stably even with less regularization.
Due to space limitations, we defer details and additional results to Appendix \ref{sec:empirical_robustness}, and only show an illustrative example here. Figure \ref{fig:mnist_workshop} shows results on MNIST where the discriminator's feedback is perturbed with probability $p=0$ (left) and $p=0.3$ (right).  
\begin{figure}[htp]
\vspace{-0.1in}
 \centering
   \includegraphics[width=2.5in]{mnist_ws}
   \vspace{-0.1in}
   \caption{Empirical Results on MNIST. The original GAN (top row) collapses to an undesired mode in the presence of perturbations (right column), whereas the robust GAN (bottom row) still learns well.}\label{fig:mnist_workshop} %\sj{dots in the legend are very hard to see. can you make them bigger?}}\label{fig:guassian_gan_005}
   \vspace{-0.1in}
 \end{figure}
Clearly, the standard GAN (first row) is heavily affected by the attack – it learns the data distribution without attack but fails once erroneous feedbacks are present. In contrast, the Piece\_GAN (second row), a robust model by Framework 2, still performs well as predicted theoretically.
 }

%\blue{\emph{Remark:}
Inspired by our theoretical results, in Appendix \ref{sec:empirical_edge}
 we further extend our framework and obtain a class of models that relates to and extends Wassterstein GANs, and performs well empirically.
 %}


==> intro_old.tex <==
Adversarial training of generative models~\citep{goodfellow2014generative} has been very popular in recent years and its nice formulations and superior performances have led to various applications such as realistic image generation, text to image synthesis, 3D object generation, and video prediction \citep{reed2016generative, 3dgan, vondrick2016generating}. Despite their success, such models are known to be difficult to train \cite{goodfellow2016nips}. The generator and discriminator oscillate significantly from iteration to iteration, and slight imbalances in their capacity frequently causes the training objective to diverge. 
%Another common problem suffered by GANs is \emph{mode collapse}, where the distribution learned by the generator concentrates on a few modes of the true data distribution, ignoring the rest of the space. In the case of images, this failure results in generated images that albeit realistic, lack diversity and reduce to a handful of prototypes. 
As such, there have been an actively line of research on improving the GAN training~\citep{radford2015unsupervised,nowozin2016f,goodfellow2016nips,salimans2016improved,arjovsky2017wasserstein,gulrajani2017improved,arjovsky2017towards,huang2017stacked,zhao2016energy,miyato2018spectral,karras2018progressive,durugkar2017generative,bora2018ambientgan:}. 

Most existing work aims at improving among three directions: formulations~(objective functions), network architectures, and training dynamics. For example, one could derive other objective functions based on different divergence measures between probability distributions \cite{nowozin2016f,arjovsky2017wasserstein}; include multiple discriminators or generators in the hope that multiple sources could lead to more stable behavior \cite{durugkar2017generative,tolstikhin2017adagan,nguyen2017dual}; or try to devise algorithms that better regularize the training process \cite{salimans2016improved,gulrajani2017improved,uehara2016generative,karras2018progressive}. 

This work falls into the first category, where the goal is to formulate objective functions in a principled manner. However, unlike most of the existing works focusing on divergence measures, our inquiry is that it is possible that the empirical instability of GAN could be caused by internally lacking of ``robustness'' under some meaningful notion. The two-player non-convex setting complicates the overall optimization process and such lacking of robustness is further amplified during training. 

Robustness is an important property for machine learning applications. Many classical machine learning algorithms that are based on regularization can be reformulated as robust optimization problems, implying that robustness helps generalization \cite{sra2012optimization}. More recently, there is an increasing interest in robust classifiers due to the presence of adversarial examples \cite{szegedy2013intriguing,goodfellow2014explaining}. However, to our best knowledge, robustness has not been explored in the field of designing GANs. While termed as ``adversarial networks'', many works in GAN takes a cooperative viewpoint in the sense that the discriminator freely shares information with the generator. ``From this point of view, the discriminator is more like a teacher instructing the generator in how to improve than an adversary. So far, this cooperative view has not led to any particular change in the development of the mathematics \cite{goodfellow2016nips}''. In pursing a meaningful notion of robustness, this work takes a different viewpoint. Rather than being a teacher, what if the discriminator is not ``honest'' and works more or less like an adversary? What if the information shared by the discriminator is perturbed? Such a perspective clearly differentiates us from existing works. From this new viewpoint,
could we define a consistent measure of robustness? Could we then systematically study the robustness property of GAN models? Those are the questions we try to address in this paper.

We list our contribution as follows:\\[3pt]
$\bullet\;\;$ We formulate the problem of GAN training under dishonest adversaries and introduce a notion of robustness. To the best of our knowledge, we are the first to explore such setting.\\
$\bullet\;\;$ We show in theory that GAN in its original formulation is vulnerable to dishonest adversaries. This motivates us to propose guaranteed frameworks that are robust against dishonest adversaries, with which one will successfully train a generator even with the presence of an adversary. \\
$\bullet\;\;$ We design a systematic experimental study and show that when the assumptions are approximately met, the models within our frameworks are indeed robust against adversaries. Along the way, we also explore the practical effect of one of the common regularization techniques, clipping, on our theory of robustness.


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

